Parting with Illusions about Deep Active Learning

Active learning aims to reduce the high labeling cost involved in training machine learning models on large datasets by efficiently labeling only the most informative samples. Recently, deep active learning has shown success on various tasks. However, the conventional evaluation scheme used for deep active learning is below par. Current methods disregard some apparent parallel work in the closely related fields. Active learning methods are quite sensitive w.r.t. changes in the training procedure like data augmentation. They improve by a large-margin when integrated with semi-supervised learning, but barely perform better than the random baseline. We re-implement various latest active learning approaches for image classification and evaluate them under more realistic settings. We further validate our findings for semantic segmentation. Based on our observations, we realistically assess the current state of the field and propose a more suitable evaluation protocol.

==> egbib.tex <==
@incollection{Douglas2011Algorithms,
  author = {Douglas, David H. and Peucker, Thomas K.},
  booktitle = {Classics in Cartography},
  title = {{Algorithms for the Reduction of the Number of Points Required to Represent a Digitized Line or its Caricature}},
  year = {2011}
}

%Uncertainty for neural networks
@incollection{NIPS2016_6501,
title = {Deep Exploration via Bootstrapped DQN},
author = {Osband, Ian and Blundell, Charles and Pritzel, Alexander and Van Roy, Benjamin},
booktitle = {NeurIPS},
year = {2016},
}

@incollection{NIPS2017_7219,
title = {Simple and Scalable Predictive Uncertainty Estimation using Deep Ensembles},
author = {Lakshminarayanan, Balaji and Pritzel, Alexander and Blundell, Charles},
booktitle = {NeurIPS},
year = {2017},
}

@inproceedings{Blundell:2015:WUN:3045118.3045290,
 author = {Blundell, Charles and Cornebise, Julien and Kavukcuoglu, Koray and Wierstra, Daan},
 title = {Weight Uncertainty in Neural Networks},
 booktitle = {ICML},
 year = {2015},
} 

% Dropout for uncertainty
@inproceedings{Gal:2016:DBA:3045390.3045502,
 author = {Gal, Yarin and Ghahramani, Zoubin},
 title = {Dropout As a Bayesian Approximation: Representing Model Uncertainty in Deep Learning},
 booktitle = {ICML},
 year = {2016},
}

@inproceedings{Gal2016Bayesian,
Author = {Yarin Gal and Zoubin Ghahramani},
Title = {Bayesian Convolutional Neural Networks with {B}ernoulli Approximate Variational Inference},
Year = {2016},
booktitle = {ICLR-workshop track},
}

% dropout for AL, shows results on MNIST and small medical dataset
@inproceedings{Gal:2017:DBA:3305381.3305504,
 author = {Gal, Yarin and Islam, Riashat and Ghahramani, Zoubin},
 title = {Deep Bayesian Active Learning with Image Data},
 booktitle = {ICML},
 year = {2017},

} 

% highest-entropy

@INPROCEEDINGS{5206627,
author={A. J. {Joshi} and F. {Porikli} and N. {Papanikolopoulos}},
booktitle={CVPR},
title={Multi-class active learning for image classification},
year={2009},}

@article{Wang:2017:CAL:3203306.3203314,
 author = {Wang, Keze and Zhang, Dongyu and Li, Ya and Zhang, Ruimao and Lin, Liang},
 title = {Cost-Effective Active Learning for Deep Image Classification},
 journal = {IEEE Trans. Cir. and Sys. for Video Technol.},
 year = {2017},
} 

% distance based uncertainty
@article{Tong:2002:SVM:944790.944793,
 author = {Tong, Simon and Koller, Daphne},
 title = {Support Vector Machine Active Learning with Applications to Text Classification},
 journal = {JMLR},
 year = {2002},

} 

% the power of ensemble
@InProceedings{Beluch_2018_CVPR,
author = {Beluch, William H. and Genewein, Tim and Nürnberger, Andreas and Köhler, Jan M.},
title = {The Power of Ensembles for Active Learning in Image Classification},
booktitle = {CVPR},
year = {2018}
} 

% variation ratio
@article{10.1093/sf/44.3.455,
    author = {Johnson, Elmer H.},
    title = {Elementary Applied Statistics: For Students in Behavioral Science },
    journal = {Social Forces},
    year = {1966},
    }

% representtation based AL

% Core-set approach
@inproceedings{sener2018active,
title={Active Learning for Convolutional Neural Networks: A Core-Set Approach},
author={Ozan Sener and Silvio Savarese},
booktitle={ICLR},
year={2018},
}

% learning loss
@InProceedings{Yoo_2019_CVPR,
author = {Yoo, Donggeun and Kweon, In So},
title = {Learning Loss for Active Learning},
booktitle = {CVPR},
year = {2019}
} 

% VAAL 
@InProceedings{Sinha_2019_ICCV,
author = {Sinha, Samarth and Ebrahimi, Sayna and Darrell, Trevor},
title = {Variational Adversarial Active Learning},
booktitle = {ICCV},
year = {2019}
} 

% object detection


% human pose estimation
@INPROCEEDINGS{8237730,
author={B. {Liu} and V. {Ferrari}},
booktitle={ICCV},
title={Active Learning for Human Pose Estimation},
year={2017},}

% AL for semantic segmentation
@INPROCEEDINGS{7780682,
author={S. D. {Jain} and K. {Grauman}},
booktitle={CVPR},
title={Active Image Segmentation Propagation},
year={2016},}

% suggestive annotation

@inproceedings{SA,
  author    = {Lin Yang and
               Yizhe Zhang and
               Jianxu Chen and
               Siyuan Zhang and
               Danny Z. Chen},
  title     = {Suggestive Annotation: {A} Deep Active Learning Framework for Biomedical
               Image Segmentation},
  booktitle = {Medical Image Computing and Computer Assisted Intervention - {MICCAI}},
  year      = {2017},
}

% CEREALS 
@inproceedings{Mackowiak2018CEREALSC,
  title={CEREALS - Cost-Effective REgion-based Active Learning for Semantic Segmentation},
  author={Radek Mackowiak and Philip Lenz and Omair Ghori and Ferran Diego and Oliver Lange and Carsten Rother},
  booktitle={BMVC},
  year={2018}
}

% SSL for image classification
@incollection{NIPS2017_6719,
title = {Mean teachers are better role models: Weight-averaged consistency targets improve semi-supervised deep learning results},
author = {Tarvainen, Antti and Valpola, Harri},
booktitle = {NeurIPS},
year = {2017},
}

@article{Xie2019UnsupervisedDA,
  title={Unsupervised Data Augmentation for Consistency Training},
  author={Xie, Qizhe and Dai, Zihang and Hovy, Eduard and Luong, Minh-Thang and Le, Quoc V},
  journal={arXiv preprint arXiv:1904.12848},
  year={2019}
}

@InProceedings{Zhai_2019_ICCV,
author = {Zhai, Xiaohua and Oliver, Avital and Kolesnikov, Alexander and Beyer, Lucas},
title = {S4L: Self-Supervised Semi-Supervised Learning},
booktitle = {ICCV},
year = {2019}
} 

@inproceedings{conf/iclr/LaineA17,
  author = {Laine, Samuli and Aila, Timo},
  booktitle = {ICLR (Poster)},
  title = {Temporal Ensembling for Semi-Supervised Learning.},
  year = 2017
}


@ARTICLE{8417973,
author={T. {Miyato} and S. {Maeda} and M. {Koyama} and S. {Ishii}},
journal={TPAMI},
title={Virtual Adversarial Training: A Regularization Method for Supervised and Semi-Supervised Learning},
year={2019},}


@inproceedings{
athiwaratkun2018there,
title={There Are Many Consistent Explanations of Unlabeled Data: Why You Should Average},
author={Ben Athiwaratkun and Marc Finzi and Pavel Izmailov and Andrew Gordon Wilson},
booktitle={ICLR},
year={2019},
}

@inproceedings{
ssl_al,
title={Consistency-Based Semi-Supervised Active Learning: Towards Minimizing Labeling Budget},
author={Anonymous},
booktitle={Submitted to ICLR},
year={2020},
url={https://openreview.net/forum?id=HJl8SkBYPr},
note={under review}
}


@inproceedings{
rethinking_al,
title={Rethinking deep active learning: Using unlabeled data at model training},
author={Anonymous},
booktitle={Submitted to ICLR},
year={2020},
url={https://openreview.net/forum?id=rJehllrtDS},
note={under review}
}


% semi-supervised consistency regularization
@article{DBLP:journals/corr/abs-1906-01916,
  author    = {Geoffrey French and
               Timo Aila and
               Samuli Laine and
               Michal Mackiewicz and
               Graham D. Finlayson},
  title     = {Consistency regularization and CutMix for semi-supervised semantic
               segmentation},
  journal   = {CoRR},
  year      = {2019},
}

@InProceedings{Kalluri_2019_ICCV,
author = {Kalluri, Tarun and Varma, Girish and Chandraker, Manmohan and Jawahar, C.V.},
title = {Universal Semi-Supervised Semantic Segmentation},
booktitle = {ICCV},
year = {2019}
}

%s4GAN
@article{1908.05724,
Author = {Sudhanshu Mittal and Maxim Tatarchenko and Thomas Brox},
Title = {Semi-Supervised Semantic Segmentation with High- and Low-level Consistency},
journal = {arXiv preprint arXiv:1908.05724},
Year = {2019},
}

% Hung et al
@inproceedings{Hung_semiseg_2018,
  author = {W.-C. Hung and Y.-H. Tsai and Y.-T. Liou and Y.-Y. Lin and M.-H. Yang},
  booktitle = {BMVC},
  title = {Adversarial Learning for Semi-supervised Semantic Segmentation},
  year = {2018}
}

@incollection{NIPS2014_5423,
title = {Generative Adversarial Nets},
author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {NeurIPS},
year = {2014},
}

% Realistic eval of SSL
@incollection{NIPS2018_7585,
title = {Realistic Evaluation of Deep Semi-Supervised Learning Algorithms},
author = {Oliver, Avital and Odena, Augustus and Raffel, Colin A and Cubuk, Ekin Dogus and Goodfellow, Ian},
booktitle = {NeurIPS},
year = {2018},
}

% autoaugment
@InProceedings{Cubuk_2019_CVPR,
author = {Cubuk, Ekin D. and Zoph, Barret and Mane, Dandelion and Vasudevan, Vijay and Le, Quoc V.},
title = {AutoAugment: Learning Augmentation Strategies From Data},
booktitle = {CVPR},
year = {2019}
} 

% cutout
@article{devries2017cutout,  
  title={Improved Regularization of Convolutional Neural Networks with Cutout},  
  author={DeVries, Terrance and Taylor, Graham W},  
  journal={arXiv preprint arXiv:1708.04552},  
  year={2017}  
}

@inproceedings{mscoco,
    title = {Microsoft {COCO}: Common Objects in Context},
    author = {Tsung-Yi Lin and Michael Maire and Serge Belongie and James Hays and Pietro Perona and Deva Ramanan and Piotr Dollár and C. Lawrence Zitnick},
    booktitle = {ECCV},
    year = {2014},
}

@article{DBLP:journals/pami/ChenPKMY18,
  author    = {Liang{-}Chieh Chen and George Papandreou and Iasonas Kokkinos and Kevin Murphy and Alan L. Yuille},
  title     = {DeepLab: Semantic Image Segmentation with Deep Convolutional Nets, Atrous Convolution, and Fully Connected CRFs},
  journal   = {TPAMI},
  year      = {2018},
  }
  
  @article{pascal_voc,
 author = {Everingham, Mark and Gool, Luc and Williams, Christopher K. and Winn, John and Zisserman, Andrew},
 title = {The Pascal Visual Object Classes (VOC) Challenge},
 journal = {IJCV},
 year = {2010},
} 

@InProceedings{Benenson_2019_CVPR,
author = {Benenson, Rodrigo and Popov, Stefan and Ferrari, Vittorio},
title = {Large-Scale Interactive Object Segmentation With Human Annotators},
booktitle = {CVPR},
year = {2019}
} 

@InProceedings{Aghdam_2019_ICCV,
author = {Aghdam, Hamed H. and Gonzalez-Garcia, Abel and Weijer, Joost van de and Lopez, Antonio M.},
title = {Active Learning for Deep Detection Neural Networks},
booktitle = {ICCV},
year = {2019}
} 

@INPROCEEDINGS{6907021,
author={R. {Paul} and D. {Feldman} and D. {Rus} and P. {Newman}},
booktitle={ICRA},
title={Visual precis generation using coresets},
year={2014},}


@INPROCEEDINGS{Zagoruyko2016WRN,
    author = {Sergey Zagoruyko and Nikos Komodakis},
    title = {Wide Residual Networks},
    booktitle = {BMVC},
    year = {2016}}
    
    

@InProceedings{pmlr-v32-houlsby14,
  title = 	 {Cold-start Active Learning with Robust Ordinal Matrix Factorization},
  author = 	 {Neil Houlsby and Jose Miguel Hernandez-Lobato and Zoubin Ghahramani},
  booktitle = {ICML},
  year = 	 {2014},

}


@InProceedings{mixmatch,
author = {Berthelot, David and Carlini, Nicholas and Goodfellow, Ian and Papernot, Nicolas and Oliver, Avital and Raffel, Colin},
year = {2019},
booktitle = {NeurIPS},
title = {MixMatch: A Holistic Approach to Semi-Supervised Learning}
}


@article{paszke2017automatic,
  title={Automatic differentiation in PyTorch},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  booktitle={NIPS Workshops},
  year={2017}
}

@inproceedings{visionUncertainties,
   author = {Alex Kendall and Yarin Gal},
   title = "{What Uncertainties Do We Need in Bayesian Deep Learning for Computer Vision?}",
   booktitle = {NeurIPS},
   year = {2017}
}


@inproceedings{ravanbakhsh:MIDLAbstract2019a,
title={Uncertainty-Driven Semantic Segmentation through Human-Machine Collaborative Learning},
author={Mahdyar Ravanbakhsh and Tassilo Klein and Kayhan Batmanghelich and Moin Nabi},
booktitle={International Conference on Medical Imaging with Deep Learning -- Extended Abstract Track},
year={2019}
}


@inproceedings{Seung:1992:QC:130385.130417,
 author = {Seung, H. S. and Opper, M. and Sompolinsky, H.},
 title = {Query by Committee},
 booktitle = {Annual Workshop on Computational Learning Theory},
 year = {1992},
} 


@article{Shannon1948,
  author = {Shannon, Claude Elwood},
  journal = {The Bell System Technical Journal},
  title = {A Mathematical Theory of Communication},
  year = 1948
}

@inproceedings{
anonymous2020semisupervised,
title={Semi-supervised semantic segmentation needs strong, high-dimensional perturbations},
author={Anonymous},
booktitle={Submitted to ICLR},
year={2020},
url={https://openreview.net/forum?id=B1eBoJStwr},
note={under review}
}
